Scattering-matrix approach for a quantitative evaluation of the topological protection in valley photonic crystals

In this work, we use valley-topological triangular resonators coupled to an input waveguide to evaluate the quality of the topological protection. To that purpose, we first analyze via numerical simulations the existence of backward scattering at cavity corners or transmission with pseudo-spin conversion at the splitter between the input waveguide and the cavity. We evidence that a breakdown of topological protection takes place, in particular at sharp corners, which results in transmission minima and split-resonances, otherwise non-existent. In order to evaluate the small coupling coefficients associated to this breakdown, a phenomenological model based on an exact parameterization of scattering matrices at splitters and corners of the resonators is then introduced. By comparison with the numerical simulations, we are able to quantify the loss of topological protection at sharp bends and splitters. Finally, we use the obtained set of phenomenological parameters to compare the predictions of the phenomenological model with full numerical simulations for fractal-inspired cavities based on the Sierpi\'nski triangle construction. We show that the agreement is overall good, but shows more differences for the cavity composed of the smallest triangles. Our results suggest that even in a system exempt of geometrical and structural defects, topological protection is not complete at corners, sharp bends and splitters. However, simpler but predictive calculations can be realized with a phenomenological approach, allowing simulations of very large devices beyond the reach of standard simulation methods, which is crucial to design photonic devices which gather compactness and low losses through topological conduction of electromagnetic waves.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
